Empirical Understanding of Deletion Privacy: Experiences, Expectations, and Measures

Social platforms are heavily used by individuals to share their thoughts and personal information. However, due to regret over time about posting inappropriate social content, embarrassment, or even life or relationship changes, some past posts might also pose serious privacy concerns for them. To cope with these privacy concerns, social platforms offer deletion mechanisms that allow users to remove their contents. Quite naturally, these deletion mechanisms are really useful for removing past posts as and when needed. However, these same mechanisms also leave the users potentially vulnerable to attacks by adversaries who specifically seek the users' damaging content and exploit the act of deletion as a strong signal for identifying such content. Unfortunately, today user experiences and contextual expectations regarding such attacks on deletion privacy and deletion privacy in general are not well understood. To that end, in this paper, we conduct a user survey-based exploration involving 191 participants to unpack their prior deletion experiences, their expectations of deletion privacy, and how effective they find the current deletion mechanisms. We find that more than 80% of the users have deleted at least a social media post, and users self-reported that, on average, around 35% of their deletions happened after a week of posting. While the participants identified the irrelevancy (due to time passing) as the main reason for content removal, most of them believed that deletions indicate that the deleted content includes some damaging information to the owner. Importantly, the participants are significantly more concerned about their deletions being noticed by large-scale data collectors (e.g., the government) than individuals from their social circle. Finally, the participants felt that popular deletion mechanisms are not very effective in protecting the privacy of those deletions.

==> results.tex <==
\section{Results}

% \renewcommand{\figurewidth}{0.5}
% \renewcommand{\figurescale}{0.45}
% \begin{figure*}[t]%
% 	%\centering
% 	\begin{subfigure}{\figurewidth\textwidth}
% 		\includegraphics[scale=\figurescale]{figures/platformUsage.pdf}
% 		\caption{Usage pattern\label{fig:platform_usage} }
% 	\end{subfigure}
% 	~~~
% 	\begin{subfigure}{\figurewidth\textwidth}
% 	   \includegraphics[scale=\figurescale]{figures/deletionPlatforms.pdf}
% 	   \caption{Previous and future deletions\label{fig:platform_deletion} }
% 	\end{subfigure}
% 	\caption{On the left the usage pattern (in percentage) of different social platforms by the participants. On the right the previous and possible future deletions from each social platform. The numbers present the percentage of the participants that answered the corresponding question.}
%     \label{fig:platform_usage_deletion}
% \end{figure*}

%\begin{figure}
%	\centering
%	\includegraphics[scale = 0.42]{figures/platformUsage.pdf}
%	\caption{the usage pattern (in percentage) of different social platforms by the participants.}
%	\label{fig:platform_usage}
%\end{figure}





\begin{table}[tb]
    %\resizebox{\columnwidth}{!}{
        %\multicolumn{3}{c}{\textbf{Someone Noticed Their Deletion}    &               \\
        \caption{Stats}
        \begin{tabular}{lccc}
        \toprule
                                                &   \textbf{US}    &  \textbf{Europe} & \textbf{Total} \\
                                                &        \# (\%)      &  \# (\%)         &  \# (\%)    \\
        \midrule
        \multicolumn{4}{l}{\textbf{Total participants}}\\
            \quad Sections 1-3                  &   93 (49\%)      &  98 (51\%)       &   191 (100\%)  \\
            \quad Section 4                     &   84 (63\%)      &  50 (37\%)       &   134 (100\%)  \\
        \midrule
        \multicolumn{4}{l}{\textbf{Have deleted a post}}\\
            \quad Yes                           &   81 (87\%)      &  75 (76\%)       &  156 (82\%)     \\
            \quad No                            &   11 (12\%)      &  19 (19\%)       &  30 (16\%)      \\
            \quad Don't know                    &    1 (1\%)       &   4 (4\%)        &   5 (3\%)       \\
        \hline
        \multicolumn{4}{l}{\textbf{Freq of deletion after posting}}\\
            \quad within less than 2 minute     &   (22\%)      &  (27\%)       &   (24\%)     \\
            \quad within 2 minute - 1 hour      &   (15\%)      &  (18\%)       &  (16\%)      \\
            \quad within 1 - 24 hours           &   (14\%)       & (13\%)        &  (13\%)       \\
            \quad within  1 - 7 days            &   (14\%)       & (9\%)        &   (11\%)       \\
            \quad after a week                  &   (36\%)       & (34\%)        &   (35\%)       \\
        \hline
        \multicolumn{4}{l}{\textbf{Someone noticed their deletions}}\\
            \quad Yes                           &   22 (27\%)      &  32 (43\%)       &  54 (35\%)     \\
            \quad No                            &   46 (57\%)      &  36 (48\%)       &  82 (53\%)     \\
            \quad Don't know                    &   13 (16\%)      &   7 (9\%)        &  20 (13\%)       \\
        \hline  
        \multicolumn{4}{l}{\textbf{Discomforts due to the notice}}\\
            \quad Yes                           &    2 (9\%)      &   7 (22\%)       &  9 (17\%)     \\
            \quad No                            &   19 (86\%)     &  25 (78\%)       & 44 (81\%)     \\
            \quad Prefer not to say             &    1 (5\%)      &   ---            &  1 (13\%)       \\
        \hline    
        \multicolumn{4}{l}{\textbf{Noticed others' deletions}}\\
            \quad Yes                           &   61 (66\%)      &  69 (70\%)       & 130 (68\%)     \\
            \quad No                            &   31 (33\%)      &  29 (30\%)       &  60 (31\%)     \\
            \quad Don't know\qquad\qquad                &    1 (1\%)       &   0 (0\%)        &   1 (1\%)       \\
        \hline
        \multicolumn{4}{l}{\textbf{Subject of a deleted post}}\\
            \quad Yes                           &   12 (20\%)      &  20 (29\%)       & 32 (25\%)     \\
            \quad No                            &   50 (82\%)      &  49 (71\%)       & 99 (76\%)     \\
        \hline
        \multicolumn{4}{l}{\textbf{Deletion content is sensitive/damaging}}\\
            \quad Strongly agree                &   9 (10\%)      &  8 (8\%)        &  17 (9\%)     \\
            \quad Somewhat agree                &  34 (36\%)      & 47 (48\%)       &  81 (42\%)      \\
            \quad Neither agree nor disagree    &  21 (23\%)      & 24 (24\%)       &  45 (24\%)       \\
            \quad Somewhat disagree             &  20 (21\%)      & 15 (15\%)       &  35 (18\%)       \\
            \quad Strongly disagree             &   9 (10\%)      &  4 (4\%)        &  13 (7\%)       \\
        \bottomrule
        \end{tabular}
    %}
\end{table}
%
%
%
\begin{table}[h!]
    \caption{Reasons for considering deletions as sensitive/damaging}
    %\resizebox{\columnwidth}{!}{
        \begin{tabular}{lc}
        \toprule
        \textbf{Reason}    &  \textbf{\# (\%)} \\
        \midrule
        Embarrassing/inappropriate/emotional                &   80  (43\%)   \\  
        Irrelevant/factually wrong/grammar/spelling         &   49  (26\%)   \\
        Context dependent                                   &   40  (21\%)   \\
        no attention                                        &    5  (3\%)   \\
        privacy                                             &    6  (3\%)    \\
        political                                           &    4  (2\%)    \\
        job-related                                         &    2  (1\%)    \\
        racism                                              &    1  (1\%)    \\
        Other                                               &    7  (4\%)     \\
        %Total population: US:92, Europe:96, total:188
        \bottomrule
        \end{tabular}
    %}
\end{table}
\vspace{5mm}


 \vspace{5mm}
 \begin{table}[h!]
     \caption{Deletion Platforms}
     %\resizebox{\columnwidth}{!}{
         \begin{tabular}{lcc}
         \toprule
         \multirow{2}{*}{\textbf{Platform}}    & \thead{Previously Deleted\\ a Post \# (\%)} & \thead{Delete a Post\\ in Future \# (\%)}\\
         \midrule
         Facebook    &   122 (78\%)  &   21 (60\%)  \\  
         Instagram   &   71  (46\%)  &   8  (23\%)   \\
         Twitter     &   53  (34\%)  &   9  (26\%)   \\
         Youtube     &   33  (21\%)  &   5  (14\%)   \\
         Whatsapp    &   21  (13\%)  &   3  (9\%)    \\
         Snapchat    &   16  (10\%)  &   4  (11\%)   \\
         Reddit      &   15  (10\%)  &   -           \\
         Linkdin     &   9   (6\%)   &   2  (6\%)    \\
         Other       &   22          &   1           \\
         \bottomrule
         \end{tabular}
     %}
 \end{table}


\begin{table*}[h!]
    \caption{Reasons of Deletion}
    %\resizebox{\columnwidth}{!}{
        \begin{tabular}{lcc}
        \toprule
        \multirow{2}{*}{\textbf{Reasons}}    & \thead{Previously Deleted\\ a Post \# (\%)} & \thead{Delete a Post\\ in Future \# (\%)}\\
        \hline
        {Being irrelevant due to time passing}          &   100 (64\%) &   11 (31\%)  \\  
        {Fixing Spelling/Grammar/FactCheck}             &   77  (49\%) &   14  (40\%)   \\
        {Post did not get enough attention}             &   46  (29\%) &   3  (9\%)   \\
        {Cleaning up my profile for new relationship}   &   36  (23\%) &   5  (14\%)   \\
        {Cleaning up my profile for new job}            &   36  (23\%) &    \textbf{13 (37\%)}    \\
        {Removing drug/alcohol/sexual related content}  &   18  (12\%)   &   1  (3\%)    \\
        {Removing Racial/Religious/Political content}   &   15  (10\%) &   1  (3\%)   \\
        {Removing due to controversy/harassment}        &   13   (8\%)   &   ---    \\
        {Removing violence/cursing related content }    &   11  (7\%) &   2 (6\%)     \\
        {Removing embarrassing content}                 &   10   (6\%)   &   1  (3\%)    \\
        {Removing health related content}               &   8   (5\%) &   ---           \\
        {Personal reason}                               &   7   (4\%)   &   1 (3\%)    \\
        {Other}                                         &   6   (4\%)   &   1  (3\%)    \\

        \hline
        \end{tabular}
    %}
\end{table*}
\vspace{5mm}



\begin{table*}[tb]
    \caption{Social groups that noticed the participants' deletions and the social groups that participants noticed their deletions.}
    %\resizebox{\columnwidth}{!}{
        \begin{tabular}{lcc}
        \toprule
        \thead{Social Circle}    & \thead{Participants' Deletion\\ was Noticed \# (\%)} & \thead{Participant Noticed\\ Others Deletions \# (\%)}\\
        
        %\multirow{2}{*}{\textbf{Participants' Deletion\\ was Noticed}} & \multicolumn{1}{c|}{\textbf{Participant Noticed Others Deletions}}\\
        \midrule
		   Family member    &   22  (41\%)  &   22 (17\%)   \\
	       Friends          &   50  (93\%)  &   91 (70\%)  \\  
	        Coworkers        &   12  (22\%)  &   43 (33\%)   \\
	       Stranger         &   \textbf{5   (9\%)}   &   \textbf{55 (42\%)}   \\
	       Prefer not to say&   ---           &   2  (2\%)   \\    
        \bottomrule
        \end{tabular}
    %}
\end{table*}


%
%
%\newcolumntype{m}{>{\hsize=.6\hsize}X}
\begin{table*}[tb]
    \caption{The medium used to notice the deletions}
    %\resizebox{\columnwidth}{!}{
        \begin{tabular}{lcc}
        \toprule
        \multirow{2}{*}{\textbf{Medium}}    & \thead{Participant noticed\\ others deletions \# (\%)} & \thead{Participant's deletion\\ noticed by others \# (\%)}\\
        \midrule
        {Interaction with the post (e.g., commenting, etc.)}
                                                        &   75  (58\%) &   9 (16\%)  \\  
        {Checking user's profile proactively}           &   69  (53\%) &  27 (49\%)   \\
        {Mentioned in the users' posts (e.g., tagged in a photo)}   
                                                        &   29  (22\%) &  10 (18\%)   \\
        {Someone sent/mentioned the post to participant}&   31  (24\%) &   3 (5\%)    \\
        {Other}                                         &   3   (2\%)  &   6 (11\%)    \\
        %Total population: 130, 55
        \bottomrule
        \end{tabular}
    %}
\end{table*}




\begin{table*}[h!]
    \caption{Possible discomforts due to deletions.}
    %\resizebox{\columnwidth}{!}{
        \begin{tabular}{lc}
        \toprule
        \textbf{Possible Discomforts}    &  \textbf{\# (\%)} \\
        \midrule
        Minimum consequence                 &   59  (33\%)   \\  
        Explaining/justifying/worried       &   49  (28\%)   \\
        Publicizing/harassment/dislike      &   31  (17\%)   \\
        Embarrassment/shame/insecure        &   25  (14\%)   \\
        Loss of privacy                     &   7   (4\%)    \\
        Loss of archival value              &   2   (1\%)    \\
        Other                               &   5   (3\%)     \\
        %Total population: US:89, Europe:89, total:178
        \bottomrule
        \end{tabular}
    %}
\end{table*}
\vspace{5mm}







\begin{figure*}[t]%
	%\centering
	\begin{subfigure}{\figurewidth\textwidth}
		\includegraphics[scale=.4]{figures/likelihoodOfNoticingOhtersDeletion.pdf}
		\caption{participant noticing others' deletions\label{fig:likelihood_deletion_noticingothers} }
	\end{subfigure}
	~~~~~
	\begin{subfigure}{\figurewidth\textwidth}
	   \includegraphics[scale=0.4]{figures/likelihoodOfOthersNoticingDeletion.pdf}
	   \caption{others noticing participants deletions\label{fig:likelihood_deletion_othersnoticing} }
	\end{subfigure}
	
    \caption{Likelihood of deletion notice. On the left, the likelihood of the participant noticing the deletions of other individuals (from its social circle) is shown. On the right, the likelihood of other individuals noticing the participants deletions is shown.}
    \label{fig:likelihood_deletion}
    \vspace{-3mm}
\end{figure*}



\begin{figure*}[t]%
	%\centering
	\begin{subfigure}{0.44\textwidth}
		\includegraphics[height=7cm]{figures/ci_plots/ci_recp_sub_us.pdf}
		\caption{US\label{fig:ci_recp_sub_us} }
	\end{subfigure}
	~~~~~
	\begin{subfigure}{0.44\textwidth}
	   \includegraphics[height=7cm]{figures/ci_plots/ci_recp_sub_europe.pdf}
	   \caption{Europe \label{fig:ci_recp_sub_europe} }
	\end{subfigure}
	
    \caption{Information flows Considering only the Recipient and Subject}
    \label{fig:ci_recp_sub}
    \vspace{-3mm}
\end{figure*}


\begin{figure*}[t]%
	%\centering
	\begin{subfigure}{0.45\textwidth}
		\includegraphics[height=7cm]{figures/ci_plots/ci_recp_reason_us.pdf}
		\caption{US\label{fig:ci_recp_reason_us} }
	\end{subfigure}
	~~~~~
	\begin{subfigure}{0.45\textwidth}
	    \includegraphics[height=7cm]{figures/ci_plots/ci_recp_reason_europe.pdf}
	    \caption{Europe \label{fig:ci_recp_reason_europe} }
	\end{subfigure}
	
    \caption{Information flows Considering only the Recipient and The Attribute (Deletion Reason)}
    \label{fig:ci_recp_reason}
    \vspace{-3mm}
\end{figure*}


\begin{figure*}[t]%
	%\centering
	\begin{subfigure}{0.45\textwidth}
		\includegraphics[height=7cm]{figures/ci_plots/ci_recp_meth_us.pdf}
		\caption{US\label{fig:ci_recp_meth_us} }
	\end{subfigure}
	~~~~~
	\begin{subfigure}{0.45\textwidth}
	    \includegraphics[height=7cm]{figures/ci_plots/ci_recp_meth_europe.pdf}
	    \caption{Europe \label{fig:ci_recp_meth_europe} }
	\end{subfigure}
	
    \caption{Information flows Considering only the Recipient and The Transmission Principle (Method o noticing deletion)}
    \label{fig:ci_recp_meth}
    \vspace{-3mm}
\end{figure*}






\renewcommand{\figurescale}{0.5}
\renewcommand{\figurewidth}{0.9}

\begin{figure*}[t]%
	\centering
	\begin{subfigure}{\figurewidth\textwidth}
		\includegraphics[scale=\figurescale]{figures/solutions_effectiveness_us.pdf}
		\caption{US\label{fig:sol_effective_us} }
	\end{subfigure}\\
	
	\begin{subfigure}{\figurewidth\textwidth}
	    \includegraphics[scale=\figurescale]{figures/solutions_effectiveness_europe.pdf}
	    \caption{Europe \label{fig:sol_effective_europe} }
	\end{subfigure}\\
	
	\begin{subfigure}{\figurewidth\textwidth}
	    \includegraphics[scale=\figurescale]{figures/solutions_effectiveness_all.pdf}
	    \caption{Combined \label{fig:sol_effective_all} }
	\end{subfigure}
	
    \caption{Deletion Technique Effectiveness}
    \label{fig:sol_effective}
    \vspace{-3mm}
\end{figure*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% LIMITATIONS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Limitations}

==> survey_beforeUsenix20Rebuttal.tex <==
\newpage
\onecolumn
\section{Survey}
Below we are providing the question asked from the volunteers in the survey.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                           GENERAL SOCIAL MEDIA 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Social Media Usage \& Post Deletions}
We begin the survey with the following question asking about the users' usage of social media and whether they have ever deleted a post
\begin{enumerate}[start=1,label={\bfseries Q\arabic*:}, leftmargin=*]
    \item \textbf{Do you currently use any social media platform (either via Mobile or via Web interface)?} (Choices: Yes, No)
    If No is selected then skip to the end of survey.
    
    \item \textbf{What is the frequency at which you currently use each of the following social media platforms?} Table matrix question where the users were asked to choose one of the following choices for each of the social platforms. (Choices: daily, weekly, monthly, yearly, don't use any more, never used) (Platforms: YouTube, Facebook, Instagram, Pinterest, Snapchat, LinkdIn, Twitter, WhatsApp, Slack, Telegram, Cybersocial, Other1[text box], Other2[text box], Other3[text box]).
    
    \item \textbf{Have you ever deleted one of your social media posts in any of the previously mentioned platforms?} (Choices: Yes, No, I don't know)
\end{enumerate}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                           SOCIAL MEDIA DELETED
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hrule
\subsection{Social Media Deleted}
If the answer to the last question above is Yes, then we ask the following questions:
\begin{enumerate}[start=4,label={\bfseries Q\arabic*:}, leftmargin=*]
    \item \textbf{Which platforms did you delete your social media posts from (you may choose multiple platforms)?}
    (Choices: YouTube, Facebook, Instagram, Pinterest, Snapchat, LinkdIn, Twitter, WhatsApp, Slack, Telegram, Cybersocial, Other1[text box], Other2[text box], Other3[text box])
    
    \item \textbf{What were the reasons behind your deletion (pick as many as needed)?}
    (Choices: Spelling/Grammar issue, Cleaning up my profile for new job, Cleaning up my profile for new relationship, Political reason, Religious reason, Cultural reason, Being irrelevant due to time passing, Others (separate with comma)[text box])
    
    \item \textbf{Can you please describe one such possible scenario where you have deleted a post? (in 1-3 sentences)}
    
    \item \textbf{Please indicate below how frequently you have deleted posts after less than 1 minute of posting, within 1 minute to 1 hour of posting, within 1 hour to 12 hours of posting and etc. For each of the cases indicate the approximate percentage using the sliders and the total should add to 100.}
    (Choices: deleted within less than 1 minute, deleted within 1 min - 1 hour, deleted within 1 - 12 hours, deleted within 12 - 24 hours, deleted within  1 - 7 days, deleted within 7-30 days, deleted within 1 - 3 months, deleted within 3 - 12 months, deleted within More than a year)
    
    \item \textbf{Has anyone ever noticed any of your deletions?}
    (Choices: Yes, No, I don't know)
    
        \vspace{2mm}
        \noindent If Yes is selected for the above question.
        \begin{enumerate}[start=1,label={\bfseries Q8.\arabic*:}]
            \item \textbf{Below we put a few categories of people from your social circle. Please point out the people from each of the categories that have noticed your deletions (i.e., you were informed that they know about your deletion)? 
            You can select multiple categories.}
            (Choices: Family member, Friends, Acquaintances/Colleagues, Stranger, Others[text box])
            
            \item \textbf{Can you please describe one such scenario where some people from your social circle noticed your post deletion? (in 1-3 sentences)}
            
            \item \textbf{Did you face any issues/problems/discomforts due to others noticing your deletions?}
            (Choices: Yes, No)
            \vspace{1mm}
            \noindent If Yes is selected for the above question.
            \begin{enumerate}[start=1,label={\bfseries Q8.3.\arabic*:}]
                \item \textbf{What issues/problems/discomforts did you face due to your post deletion? (Explain in 1-3 sentences)}
            \end{enumerate}
            \noindent If Yes is NOT selected for the above question.
            \begin{enumerate}[start=1,label={\bfseries Q8.3.\arabic*:}]
                \item \textbf{If you were to delete one of your social media posts, what possible issues/problems/discomforts do you think you might face if someone notices your post deletion? (Explain in 1-3 sentences)}
            \end{enumerate}
        \end{enumerate}
        
        \vspace{2mm}
        \noindent If Yes is NOT selected for question number 8.
        \begin{enumerate}[start=1,label={\bfseries Q8.\arabic*:}]
            \item \textbf{Below we put a few categories of people from your social circle. If you were to delete any of your social media posts, please point our how likely is it that people from each of the categories will notice your deletions?}
            (Choices: Extremely unlikely, unlikely, Neutral, likely, Extremely likely)
            (Social circle: Family member, Friends, Acquaintances/Colleagues, Stranger, Others[text box])
            
            \item \textbf{If you were to delete one of your social media posts, what possible issues/problems/discomforts do you think you might face if someone notices your post deletion? (Explain in 1-2 sentences)}

        \end{enumerate}
            
\end{enumerate}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                           SOCIAL MEDIA NOT DELETED
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hrule
\subsection{Social Media Not Deleted}
If the answer to the question number 3 is NOT Yes, then we ask the following questions:
\begin{enumerate}[start=4,label={\bfseries Q\arabic*:}, leftmargin=*]
    \item \textbf{If you were to delete any of your posts in any social media platform which platform would it be (you can select multiple platforms)? }
    (Choices: YouTube, Facebook, Instagram, Pinterest, Snapchat, LinkdIn, Twitter, WhatsApp, Slack, Telegram, Cybersocial, Other1[text box], Other2[text box], Other3[text box])
    
    \item \textbf{If you were to delete any of your posts in any social media platform, what do you think the reason behind your deletion would be (pick as many as needed)?  }
    (Choices: Spelling/Grammar issue, Cleaning up my profile for new job, Cleaning up my profile for new relationship, Political reason, Religious reason, Cultural reason, Being irrelevant due to time passing, Others (separate with comma)[text box])
    
    \item \textbf{Can you please describe one such possible scenario where you might delete a post? (in 1-3 sentences)}
    
    \item \textbf{Below we put a few categories of people from your social circle. If you were to delete any of your social media posts, please point our how likely is it that people from each of the categories will notice your deletions?}
    (Choices: Extremely unlikely, unlikely, Neutral, likely, Extremely likely)
    (Social circle: Family member, Friends, Acquaintances/Colleagues, Stranger, Others[text box])

    \item \textbf{If you were to delete one of your social media posts, what possible issues/problems/discomforts do you think you might face if someone notices your post deletion? (Explain in 1-3 sentences)}
\end{enumerate}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                           SOCIAL MEDIA DELETION NOTICED
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hrule
\subsection{Social Media Deletion Noticed}
Below we ask a series of questions about the user noticing others deletions.
\begin{enumerate}[start=9,label={\bfseries Q\arabic*:}, leftmargin=*]
    \item \textbf{Have you ever noticed anyone deleting their posts? }
    (Choices: Yes, No)
    
    \vspace{2mm}
    \noindent If Yes is selected for the above question.
    \begin{enumerate}[start=1,label={\bfseries Q9.\arabic*:}]
        \item \textbf{The individual that deleted its post belongs to which of your social groups mentioned below? (you can choose multiple answers)}
        (Choices: Family member, Friends, Acquaintances/Colleagues, Stranger, Others[text box])
        
        \item \textbf{In your opinion, what was the reason for their post deletion? (You can provide multiple answers separated by comma)}
        
        \item \textbf{Were you the subject of a deleted post made by another user (e.g., your name was mentioned in the post) or had an activity (liked, comment, repost, share, etc.) around a deleted post?}
        (Choices: Yes, No)
    \end{enumerate}
    
    \vspace{2mm}
    \noindent If Yes is NOT selected for the above question.
    \begin{enumerate}[start=1,label={\bfseries Q9.\arabic*:}]
        \item \textbf{Below we are again putting a few categories of people from your social circle. What is the likelihood of you noticing any of post deletion done by people from each of the categories?}
        (Choices: Extremely unlikely, unlikely, Neutral, likely, Extremely likely)
        (Social circle: Family member, Friends, Acquaintances/Colleagues, Stranger, Others[text box])
    \end{enumerate}
    
    \item \textbf{Do you agree or disagree to the following statement: when someone deletes a social media post, it indicates that the content of that post is sensitive/damaging to that individual.}
    (Choices: Strongly agree, Somewhat agree, Neither agree nor disagree, Somewhat disagree, Strongly disagree)
    
    \item \textbf{Why do you think so? (explain in 1-3 sentences)}
\end{enumerate}






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                           CONTEXTUAL INTEGRITY
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hrule
\subsection{Social Media Deletion Noticed}
Below we ask the acceptance of some RECIPIENT noticing a user's deletion via some METHOD when somebody is the SUBJECT of the post under different scenarios. 

RECIPIENT $\in \{$anyone, your close family member, your close friend, your coworker, a third party service, the 
government$\}$

METHOD $\in \{$deletion because they stalk your profile, deletion using non-targeted data collection techniques, deletion  because they were involved in the post (e.g., they were mentioned on the post), deletion$\}$

SUBJECT $\in \{$a post that contained some information about yourself, a post that contained some information about your family members or close friends, a post that contained some information about your coworkers, a post$\}$

\begin{enumerate}[start=12,label={\bfseries Q\arabic*:}, leftmargin=*]
    \item \textbf{We are putting a few possible reasons behind post deletions in the table below (leftmost column). For each of these reasons, imagine a situation where you deleted [SUBJECT] from one of your social media accounts due to that reason. In each of these situations, please indicate how acceptable is it for you that [RECIPIENT] notices your [METHOD]? (If you can think of other reasons please enter them in the “other” labeled text boxes and answer this same question)}

    \begin{table}[!h]
        \centering
        \begin{adjustbox}{width=0.8\columnwidth,center}
        \begin{tabular}{l||c|c|c|c|c}
             &  Completely  & Somewhat & Neutral & Somewhat  & Completely \\
             &  unacceptable & unacceptable &  & acceptable & acceptable\\

             \hline
             Post did not get enough attention & & & & &\\
             Spelling/Grammar issue & & & & &\\
             Cleaning up profile for new job & & & & &\\
             Cleaning up profile for new relationship & & & & &\\
             Political reason & & & & &\\
             Religious reason & & & & &\\
             Cultural reason & & & & &\\
             Being irrelevant due to time passing & & & & &\\
             Other1[text box] & & & & &\\
             Other2[text box] & & & & &\\
             Other3[text box] & & & & &\\
        \end{tabular}
        \end{adjustbox}
    \end{table}
    

\end{enumerate}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                           DELETION MECHANISMS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hrule
\subsection{Effectiveness of Deletion Mechanisms}
In this section of the survey, we describe different mechanisms that you may use to remove your posts from social media platforms and ask questions about the usage of those mechanisms. 

\begin{enumerate}[start=13,label={\bfseries Q\arabic*:}, leftmargin=*]
    \item \textbf{Consider the scenario that a malicious third-party service (not affiliated with the platform or users) is collecting the deleted posts of users from a social media platform that you use. The third-party service's goal is to find some deleted posts that may be damaging/sensitive to the users and use them to harass or blackmail them. However, the third-party service does not have any background information on particular users (e.g., the service does not know if a particular user will consider a post stating ``I am smoking weed" or ``I cannot trust anyone" as sensitive).
    \\\\
    To protect users from this malicious third-party service, below, we state four deletion mechanisms with their benefits and drawbacks. Please state, in your opinion, how effective is each of the deletion mechanisms in deleting your damaging/sensitive posts given the above scenario.
    }
    
        % \newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
        % \newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
        % \newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
        % \begin{table}[!h]
        %     \centering
        %     \begin{adjustbox}{width=0.99\columnwidth,center}
        %     \begin{tabular}{L{11.5cm}||C{1.2cm}|C{1.2cm}|C{1.2cm}|C{1.2cm}|C{1.2cm}||C{2.cm}}
        %          %\multicolumn{1}{c}{}& \multicolumn{5}{c|}{How effective is each of the mechanisms for deleting your damaging/sensitive posts?} & Describe cases where the mechanism might be useful and/or NOT useful to you.\\
        %          %\hline
        %          &  Not Effective at all & Slightly Effective& Moderately Effective & Very Effective & Extremely Effective &  Explain in 1-3 sentences\\
    
        %          \hline
        %          \textbf{Mechanism 1:}\newline
        %          \textbf{Description:} You and other users selectively choose the posts 
        %          to delete and press a button to remove those posts from the platform
        %          (e.g., deletion on Facebook or Twitter).\newline
        %          %
        %          \textbf{Upside:} Users' total control over what posts to delete and when to delete. The platform keeps
        %          an archive of all non-deleted posts that users can visit.\newline
        %          %
        %          \textbf{Downside:} Whenever you or any other user on the platform delete a post the third-party service will
        %          know that a user wanted to remove a specific piece of content. & & & & & &\\
                
        %         \hline
        %          \textbf{Mechanism 2:}\newline
        %          \textbf{Description:}  Removing the users' posts based on a predefined expiry date or based on the fact that there is no new views/replies on the post (e.g., Snapchat, Instagram Stories, 4chan boards).\newline
        %          %
        %          \textbf{Upside:}Since all content is auto-deleted, the third-party service can't identify specific user-desired deletions.\newline
        %          %
        %          \textbf{Downside:} All the users' posts will be removed and there will be no archive of old posts in the platform. & & & & & &\\
                 
                 
        %          \hline
        %          \textbf{Mechanism 3:}\newline
        %          \textbf{Description:}  You and other users can delete posts just like Mechanism 1. However, the platform also periodically hides and reveals non-deleted posts. The third-party service cannot view a non-deleted post while it is hidden. So a non-deleted post will be periodically viewable/non-viewable to the third-party.\newline
        %          %
        %          \textbf{Upside:} The malicious third-party cannot immediately decide if a non-viewable post is hidden by the platform or deleted by the user. This inability of the third-party service to decide is guaranteed for a limited amount of time (e.g., for up to 3 months after deletion).\newline
        %          %
        %          \textbf{Downside:}The non-deleted posts will be non-viewable to other users for some amount of time (e.g., on average 2.5 hours per day). & & & & & &\\
                
                
        %         \hline
        %          \textbf{Mechanism 4:}\newline
        %          \textbf{Description:}  The users collaborate to create a pool of non-sensitive/non-damaging decoy posts. Whenever a user deletes a damaging/sensitive post, the platform also selects a few other "similar'' looking non-sensitive/non-damaging decoy posts from this pool and delete them.\newline
        %          %
        %          \textbf{Upside:} The malicious third-party cannot decide if a deleted post is intentionally deleted by the user or deleted by the platform (chosen from the pool of non-sensitive decoy posts).\newline
        %          %
        %          \textbf{Downside:}There should be enough collaborating users and enough "similar'' non-sensitive decoy posts for each user intended deletion. & & & & & &\\
        %          \hline
        %     \end{tabular}
        %     \end{adjustbox}
        % \end{table}
    
    
    \item \textbf{Can you think of any other mechanism that can protect user deletions in presence of the malicious third-party service mentioned above? (Explain in 1-3 sentences)}
    
    
    \item \textbf{How important is it for you in general that any other user does NOT detect when you delete a particular post?}
    (Choices: Extremely important, Very important, Neutral, Slightly important, Not at all important)
    
    \item \textbf{Please explain your choice in 1-3 sentences.}
    
    \item \textbf{How important is it for you that your any and all social media posts that you ever made are always viewable for you?}
    (Choices: Extremely important, Very important, Neutral, Slightly important, Not at all important)
    
    \item \textbf{Please explain your choice in 1-3 sentences.}
    
    \item \textbf{How important is it for you that your any and all social media posts that you ever made are always viewable for the people who have permission to view the posts?}
    (Choices: Extremely important, Very important, Neutral, Slightly important, Not at all important)
    
    \item \textbf{Please explain your choice in 1-3 sentences.}


    \item Recall the third deletion mechanism explained in the previous page:\\
    Description: The platform periodically hides and reveals non-deleted posts. The third-party service cannot view a non-deleted post while it is hidden. So a non-deleted post will be periodically viewable/non-viewable to the third-party.\\ 
    Upside: The malicious third-party cannot immediately decide if a non-viewable post is hidden by the platform or deleted by the user. This inability of the third-party service to decide is guaranteed for a limited amount of time (e.g., for up to 3 months after deletion)\\
    Downside: The non-deleted posts will be non-viewable to other users for some amount of time (e.g., on average 2.5 hours per day).\\
    \textbf{Is it acceptable for you that a platform deploys this deletion mechanism? Now, some of your non-deleted posts will be be non-viewable to other users for a small amount of time in exchange for the feature that a malicious third-party service cannot immediately decide if a non-viewable post is hidden by the platform or deleted by you.}
    (Choices: Definitely yes, Probably yes, Might or might not, Probably not, Definitely not)
    
    \item \textbf{Please explain your choice in 1-3 sentences.}

    \item \textbf{Now consider a slight modification of third deletion mechanism. Imagine, the hiding/revealing part of the mechanism will only be applied to a post after a user-specified time T has passed. In this modification, within time T of publishing, a non-deleted post will be always viewable by other users (unless you delete them) and these users can interact (via views, reposts, likes, replies, etc ...) with the post just like they do today. Will this modified mechanism be more or less acceptable than the original third deletion mechanism?}
    (Choices: A lot More acceptable, Slightly more acceptable, Neutral, Slightly less acceptable, Lot less acceptable, This modification is not acceptable to me)
    
    \vspace{2mm}
    \noindent If A lot More acceptable or Slightly more acceptable is selected for the above question.
    \begin{enumerate}[start=1,label={\bfseries Q23.\arabic*:}]
        \item \textbf{Please indicate a suitable time T for the modified third deletion mechanism explained in the previous question. (you can choose multiple answers)}
        (Choices: From the post creation, After an hour, After 12 hours, After 24 hours, After 2 days, After a week, After a month or more)
        
        \item \textbf{Please explain your choice in 1-3 sentences.}
    \end{enumerate}
    
    \item Recall the fourth deletion mechanism explained in the previous section:\\
    Description: The users collaborate to create a pool of non-sensitive/non-damaging decoy posts. Whenever a user deletes a damaging/sensitive post, the platform also selects a few other "similar'' looking non-sensitive/non-damaging decoy posts from this pool and delete them.\\
    Upside: The malicious third-party cannot decide if a deleted post is intentionally deleted by the user or deleted by the platform (chosen from the pool of non-sensitive decoy posts).\\
    Downside: There should be enough collaborating users and enough "similar'' non-sensitive decoy posts for each user intended deletion. 
    \textbf{Would you be willing to offer some of your non-sensitive/non-damaging posts to be added to the decoy pool in order to protect the sensitive/damaging deletions of other users?}
    (Choices: Definitely yes, Probably yes, Might or might not, Probably not, Definitely not)
    
    \item \textbf{Please explain your choice in 1-3 sentences.}

    \item \textbf{Are you willing to offer some of your non-sensitive/non-damaging posts to the decoy pool at the time of deleting one of your sensitive/damaging posts (as cost of using the pool)?\\ 
    Existing posts from the decoy pool will be used to hide your deletion (as described in mechanism four) and your offered posts will be used for hiding future deletions of other users.}
    (Choices: Definitely yes, Probably yes, Might or might not, Probably not, Definitely not)
    
    \item \textbf{Please explain your choice in 1-3 sentences.}

    \item \textbf{Would it be acceptable for you if a social media platform (e.g., Twitter, Facebook) automatically publishes a random post on your profile. At a later time (minutes to months) the platform delete the post to protect your and other users' sensitive/damaging deletions?}
    (Choices: Definitely yes, Probably yes, Might or might not, Probably not, Definitely not)
    
    \item \textbf{Please explain your choice in 1-3 sentences.}

    \item \textbf{Would it be acceptable for you if a social media platform (e.g., Twitter, Facebook) automatically publishes a post on your profile where the post is similar to the posts that you already have on your profile. At a later time (minutes to months) the platform deletes the post to protect your and other users' sensitive/damaging deletions?}
    (Choices: Definitely yes, Probably yes, Might or might not, Probably not, Definitely not)
    
    \item \textbf{Please explain your choice in 1-3 sentences.}
            
\end{enumerate}



==> survey_instrument.tex <==
%%%%%%Introduction%%%%%%%
\vspace{2mm}
\paragraph{Introduction}
In the first step, we explain to each participant the purpose of and reason for the study as well
as the task they will be asked to do.
Moreover, we inform them how long their participation will approximately take, 
what the reward for their participation will be and that no personal data will be collected.
We further, ask the participants to have audio capabilities as there will be some videos that they will be listing to and answering questions based on them.

The survey is proceeded by users consenting to the mentioned information. 
At the end of this section to ensure that the users have some familiarity with the social platforms we ask the participants: ``Do you currently use any social media platform (e.g., Facebook, Twitter, Snapchat, Youtube, etc.), either via Mobile or via Web interface?''.
We end the survey for the participants that answer ``No'' to the question without any compensation as we state this requirement in the description of the survey.
The consent form and instructions avoided any mention of privacy or security.


%%%%%%Social media usage and post deletion%%%%%%%
\vspace{2mm}
\paragraph{Social media usage and post deletion (RQ1)}
This section of the survey was divided into four blocks.
The first \textit{general block} consists of two question about the usage frequency of different social platforms (e.g., Facebook, Twitter, Instagram, etc.) and whether the users have ever deleted one of their posts on any of the social platforms. 
Based on their answer to the deletion question one of the next two blocks were shown to them.

The \textit{deleted block} consists of \todo{six} questions, starting with asking the participants which of the platforms they have deleted their post(s) from. 
Next, they are asked about the reason behind their deletion given multiple choices (taken from~\cite{zhou2016tweet}, e.g., cleaning up profile for new job, removing drug/alcohol related content, fixing spelling/grammar issues, etc.) and allowing them to explain other reasons if needed. Next we ask about the frequency of the posts deletions within different periods (e.g., what percentage of your deletions happen within less than 2 minute of publishing?).
The next question asks the participants if they have ever become aware of someone noticing that they have deleted a post.
If they answer yes, then we ask who were the individual(s) that have noticed their deletions and if they faced any issues, problems, or discomforts due to others noticing their deletions.
Otherwise, we ask the likelihood of different social circles\todo{cite} (i.e., family members, friends, coworkers, strangers) of the participant noticing their deletions, and further allow them to explain about possible issues, problems or discomforts that they may face. 

The \textit{non-deleted block} consists of \todo{four} questions about potential deletions that users may have in the future.
The first and second question asks the participants about the platform that they may deleted their post from and for what reason given multiple choices (taken from~\cite{zhou2016tweet}, e.g., cleaning up profile for new job, removing drug/alcohol related content, fixing spelling/grammar issues, etc.) and allowing them to explain other reasons if needed.
Finally, we ask the likelihood of different social circles \todo{cite} (i.e., family members, friends, coworkers, strangers) of the participant noticing their deletions, and further allow them to explain about possible issues, problems or discomforts that they may face.

The final block in this section of the survey is the \textit{deletion noticed block}, where a series of questions about the participant noticing other peoples' deletions are asked.
The first question in this block is: ``Have you ever noticed anyone deleting their posts?'', and according the response the next set of questions are shown to the participant.
If the answer is yes, then the we ask whose deletion did they have noticed (i.e, family member, friends, coworker, stranger or others) and follow with the question of how did they become aware of the deletion(s) given some possible choices (e.g., being mentioned on the post, someone sending or mentioning the post to them, interacting with the post by liking or commenting or sharing, and checking the users' profile regularly) and allowing for explanation on other methods.
If the answer is no, then we ask the likelihood of them noticing the deletions of different individuals from their social groups (i.e, family member, friends, coworker, stranger or others).  

To see if the participants consider deleted post to contain any damaging contents, in the last question of the block we ask: ``Do you agree or disagree to the following statement: when someone deletes a social media post, it indicates that the content of that post is sensitive/damaging/embarrassing to that individual.''


%%%%%%CI-based questionnaire about deletions in different scenarios%%%%%%%
\begin{table*}[t]
    \resizebox{\textwidth}{!}{
        \begin{tabular}{|l|l|}
            \hline
            \textbf{Sender}                                                  & \textbf{Transmission Principle}                                              \\
            user itself                                                      &  because they were checking/observing your user profile regularly    \\ \cline{1-1}
            \textbf{Subject}                                                 &  because they were mentioned in the post or interacted with the post \\
            that contained some information about yourself            & \textit{null}                                                                     \\ \cline{2-2} 
            that contained some information about your family members & \textbf{Attributes}                                                          \\
            that contained some information about your friends        & Post did not get enough attention                                            \\
            that contained some information about your coworkers      & Fixing Spelling/Grammar                                                      \\
            \textit{null}                                                           & Cleaning up profile for new job                                              \\ \cline{1-1}
            \textbf{Recipient}                                               & Cleaning up profile for new relationship                                     \\
            your family member                                               & Racial/Religious/Political reason                                            \\
            your friend                                                      & Being irrelevant due to time passing                                         \\
            your coworker/acquaintance                                       & Removing sexual content                                                      \\
            a company                                                        & Removing drug/alcohol related content                                        \\
            the government                                                   & Removing violence/cursing related content                                    \\
            anyone                                                           & Removing health related content                                              \\ \hline
            \end{tabular}
    }
    \caption{Contextual integrity parameter values selected for information flow generation}
    \label{tab:ci_infoflow}
\end{table*}

\vspace{2mm}
\paragraph{CI-based questionnaire for deletions in different scenarios (RQ2)}
In this section we adapt a CI-based survey method presented in previous works~\cite{apthorpe2018discovering,apthorpe2019evaluating}  to evaluate the users acceptability of others noticing their deletions. We chose this particular survey method because it is previously tested, scalable to large respondent populations, and easily adaptable to our domain of deletion privacy. 
As mentioned in~\cref{sec:ci_background} the information transfers (``flows'') are defined according to CI as sets of five parameters: sender, subject, recipient, transmission principle and attributes.
We select lists of values for each of these parameters shown in~\cref{tab:ci_infoflow} and further explained below. 

For each deletion, the sender of the information flow will be the user itself. 
However, the subject of the post could be about anyone. In this work, we consider the social circles from~\todo{cite} where we consider five different subject categories---i) the user itself, ii) family members of the user, iii) friends of the user, iv) coworkers/acquaintance of the user, and v) anyone.

The recipient of the deletion is the individual that notices the user's deletion. Here, similar to the subject of the post we include the user's social circle with the addition of two other recipients--- a company that collects and archives the deletions of the users for a potential use in the future and the government that may use the contents of the deletions to protect the society (e.g., potential terrorist attacks) or in a opposite case use them against the citizens of the country (e.g., punishing the citizens in an authoritarian regime). 

The transmission principle of a information flow in a deletion is the method that a recipient uses to discover the deletion. We consider three discovery methods---i) discovery due to checking/observing the user profile regularly to observe any change in the user's profile (we have avoided using the term stalking due to \todo{?} and opted for its loose definition), ii) discovery due to an interaction with the post (e.g., liking, commenting, reposting, sharing, etc.), iii) discovering using any method.

There are a variety of attributes that can be associated with a post deletion. We consider the reason of the deletion to be the attribute in the information flow. 
Zhou et al.~\cite{zhou2016tweet} have taken regrettable deleted tweets and categorized them into different groups (e.g., job, sexual, alcohol, drug, cursing, relationship, health, race and religion, violence). We adapt the categories from~\cite{zhou2016tweet} and added ``fixing spelling/grammar'' from the previous work~\cite{almuhimedi2013tweets} where they shown that 18\% of deletions in Twitter are because of spelling, grammar, and spam problems.
Further we added two other reasons---``post did not get enough attention'' and ``being irrelevant due to time passing'' as suggested by our pilot participants. 

Using these values, we generate a combinatorial number of information flow for the acceptability of noticing users' deletions. 
In total there are 900 information flows that have to be labeled by the participants. 
Although it will be ideal to have all these flows to be labeled by each of the participants it is cumbersome as this section is only part of the entire survey.
To simplify the task for the participants, in the beginning of the survey the participants are randomly assigned a \textit{subject}, a \textit{transmission principle}, and three \textit{recipients}. 
For each of the assigned recipients, a Likert scale multiple choice matrix question is presented to the participants\todo{figure}.

Each individual multiple choice question in the matrices asked respondents to rate the acceptability of a single information flow on a scale of five Likert items: Completely Acceptable (2), Somewhat Acceptable (1), Neutral (0), Some- what Unacceptable (-1), Completely Unacceptable (-2).
The question text is as follow: ``We are putting a few possible reasons behind post deletions in the table below (leftmost column). For each of these reasons, imagine a situation where you deleted a post [\textit{subject}] from one of your social media accounts due to that reason. 
In each of these situations, please indicate how acceptable is it for you that [\textit{recipient}] notices your deletion [\textit{transmission principle}]?''
As a result each participant labeled three CI related question with a total of 30 flows.






%%%%%%efficiency of different deletion techniques%%%%%%%
\vspace{2mm}
\paragraph{Efficiency of different deletion techniques in protecting users deletions (RQ3)}
In this section of the survey 

